Multidimensional Manhattan Sampling and Reconstruction

This paper introduces Manhattan sampling in two and higher dimensions, and proves sampling theorems. In two dimensions, Manhattan sampling, which takes samples densely along a Manhattan grid of lines, can be viewed as sampling on the union of two rectangular lattices, one dense horizontally, being a multiple of the fine spacing of the other. The sampling theorem shows that images bandlimited to the union of the Nyquist regions of the two rectangular lattices can be recovered from their Manhattan samples, and an efficient procedure for doing so is given. Such recovery is possible even though there is overlap among the spectral replicas induced by Manhattan sampling. In three and higher dimensions, there are many possible configurations for Manhattan sampling, each consisting of the union of special rectangular lattices called bi-step lattices. This paper identifies them, proves a sampling theorem showing that images bandlimited to the union of the Nyquist regions of the bi-step rectangular lattices are recoverable from Manhattan samples, and presents an efficient onion-peeling procedure for doing so. Furthermore, it develops a special representation for the bi-step lattices and an algebra with nice properties. It is also shown that the set of reconstructable images is maximal in the Landau sense. While most of the paper deals with continuous-space images, Manhattan sampling of discrete-space images is also considered, for infinite, as well as finite, support images.

==> fig_bandlimitations.tex <==
\begin{figure*}[!t] \centerline{ 
  %
  \subfloat[]{\includegraphics[width=2in]{2dGridSpectra}}
  %
  \hfil
  %
  \subfloat[]{\includegraphics[width=2in]{3dGridSpectra2}}
  %
  \hfil
  %
  \subfloat[]{\includegraphics[width=2in]{3dPlanesSpectra2}}} 
  %
  \caption{Frequency support $\M(\Gamma)$ of Manhattan bandlimited functions.
  The frequency axes are not shown for clarity, though it should be noted that
  each support region is centered at ${\bm \u = 0}$ in the frequency domain.
  (a) Recoverable region for a Manhattan set in two dimensions corresponding to
  $\Gamma = \{ \{1\}, \{2\}\}$. (b) In three dimensions, the recoverable region
  for Manhattan lines $\Gamma = \{ \{1\},\{2\},\{3\}\}$.  (c) Also in three
  dimensions, the recoverable region for Manhattan facets $\Gamma = \{
  \{1,2\},\{2,3\},\{1,3\}\}$.  }
  %
  \label{fig:bandlimitations} 
  %
\end{figure*}



==> fig_lattices.tex <==
\begin{figure*}[!t] \centerline{ 
  %
  \subfloat[]{\includegraphics[width=2in]{lattice}%
  \label{fig:fineGridWithManhattan}}
  %
  \hfil
  %
  \subfloat[]{\includegraphics[width=2in]{lattice}%
  \label{fig:3dGridLattice}}
  %
  \hfil
  %
  \subfloat[]{\includegraphics[width=2in]{lattice}%
  \label{fig:3dPlanesLattice}}
  %
  } % end centerline
  %
  \caption{Examples of Manhattan sampling.  All circles represent points on the
  fine lattice $L(\Gamma)$, while dark circles represent sampled points on the
  Manhattan sampling structure $M(\Phi)$.  In each example,
  $\Lambda_i=4\lambda_i$ for all $i$.  (a) A Manhattan grid
  in two dimensions, corresponding to $N=2$, $\Phi = \{ \{1\}, \{2\}\}$, (b) A
  Manhattan grid in three dimensions, corresponding to $N=3$, $\Phi = \{
  \{1\},\{2\},\{3\}\}$.  (c) Manhattan facets in three dimensions,
  corresponding to $N=3$, $\Phi = \{ \{1,2\},\{2,3\},\{1,3\}\}$.  }
  %
  \label{fig:lattices} 
  %
\end{figure*}


